Federated Spectral Graph Transformers Meet Neural Ordinary Differential Equations for Non-IID Graphs

Graph Neural Network (GNN) research is rapidly advancing due to GNNs' capacity to learn distributed representations from graph-structured data. However, centralizing large volumes of real-world graph data for GNN training is often impractical due to privacy concerns, regulatory restrictions, and commercial competition. Federated learning (FL), a distributed learning paradigm, offers a solution by preserving data privacy with collaborative model training. Despite progress in training huge vision and language models, federated learning for GNNs remains underexplored. To address this challenge, we present a novel method for federated learning on GNNs based on spectral GNNs equipped with neural ordinary differential equations (ODE) for better information capture, showing promising results across both homophilic and heterophilic graphs. Our approach effectively handles non-Independent and Identically Distributed (non-IID) data, while also achieving performance comparable to existing methods that only operate on IID data. It is designed to be privacy-preserving and bandwidth-optimized, making it suitable for real-world applications such as social network analysis, recommendation systems, and fraud detection, which often involve complex, non-IID, and heterophilic graph structures. Our results in the area of federated learning on non-IID heterophilic graphs demonstrate significant improvements, while also achieving better performance on homophilic graphs. This work highlights the potential of federated learning in diverse and challenging graph settings. Open-source code available on GitHub (https://github.com/SpringWiz11/Fed-GNODEFormer).

==> section-6-Discussions.tex <==
\section{Discussions}
% In Table \ref{tab:my_label}, we present the performance of our centralized architecture across three homophilic and three heterophilic graph datasets, arranged in ascending order of dataset size. Notably, we observe significant improvements on the heterophilic graphs, alongside competitive performance on the homophilic datasets. For instance, GNODEFormer achieves the highest accuracy on the Chameleon and Squirrel datasets, with results of 79.41\% and 66.26\%, respectively. This highlights the model's strong ability to generalize in heterophilic graph scenarios. The findings suggest that GNODEFormer effectively handles heterophily, likely due to its capacity to capture more complex node relationships compared to traditional graph models like GCN and GAT, which exhibit lower performance on these datasets.

% On the homophilic datasets (Cora, CiteSeer, Photo), GNODEFormer continues to demonstrate strong results. GNODEFormer (RK-4), in particular, achieves an impressive accuracy of 95.94\% on the Photo dataset, significantly outperforming the other models. Similarly, GNODEFormer (RK-2) performs competitively on the Cora and CiteSeer datasets, showing its adaptability to homophilic graph structures. This indicates that GNODEFormer is well-suited for leveraging both heterophilic and homophilic relationships, outperforming traditional models like GCN, which struggle in heterophilic settings.

% In the federated learning setup, Tables \ref{tab:Homophilic-non-iid-for-5-clients} and \ref{tab:Heterophilic-non-iid-for-5-clients} present results for non-iid data across five clients, focusing on both homophilic and heterophilic graphs. GNODEFormer (RK-2 and RK-4) continues to excel in these distributed environments as well. In Table \ref{tab:Homophilic-non-iid-for-5-clients}, GNODEFormer (RK-4) yields the highest accuracies on the Cora, CiteSeer, and Photo datasets, with values of 89.64\%, 75.18\%, and 96.76\%, respectively, under an extreme non-iid condition (alpha = 0.01). These results emphasize the model's robustness in handling extreme non-iid scenarios on homophilic graphs in federated learning environments.

% For the heterophilic setting in Table \ref{tab:Heterophilic-non-iid-for-5-clients}, GNODEFormer (RK-4) again demonstrates superior performance, achieving 53.72\% accuracy on the Squirrel dataset. The model also performs strongly on the Chameleon and Actor datasets, with accuracies of 70.59\% and 64.22\%, respectively. These results suggest that GNODEFormer, particularly in its RK-4 configuration, is highly effective at managing non-iid data distribution across clients in federated learning scenarios, outperforming baseline models like GCN and GAT.

% Despite the strong performance demonstrated by GNODEFormer across various datasets, there are certain limitations that need to be addressed. One of the key challenges is the difficulty in achieving faster convergence on larger datasets, particularly for heterophilic graphs. This issue becomes more severe in the RK-4 configuration, where the model's complexity demands higher computational resources. As a result, training on larger datasets, especially in heterophilic settings, requires significantly more time and compute power, which may limit the model's scalability and practicality in resource-constrained environments. Future work could explore optimization techniques or more efficient architectures to mitigate these limitations while preserving the model’s strong performance.

Tables \ref{tab:my_label}, \ref{tab:Homophilic-non-iid-for-5-clients}, and \ref{tab:Heterophilic-non-iid-for-5-clients} present our model's performance on various graph datasets. GNODEFormer shows significant improvements on heterophilic graphs and competitive results on homophilic datasets. It achieves the highest accuracy on Chameleon (79.41\%) and Squirrel (66.26\%) datasets, demonstrating its ability to handle heterophily effectively. On homophilic datasets, GNODEFormer (RK-4) performs exceptionally well, achieving 95.94\% accuracy on the Photo dataset.

In federated learning setups with non-iid data across five clients, GNODEFormer continues to excel. For homophilic graphs, GNODEFormer (RK-4) achieves the highest accuracies on Cora (89.64\%), CiteSeer (75.18\%), and Photo (96.76\%) under extreme non-iid conditions. Similarly, for heterophilic graphs, it performs strongly on Squirrel (53.72\%), Chameleon (70.59\%), and Actor (64.22\%) datasets.

Despite these strengths, GNODEFormer faces challenges in achieving faster convergence on larger datasets, particularly heterophilic graphs. The RK-4 configuration requires significant computational resources, potentially limiting scalability in resource-constrained environments. Future work should address these limitations while maintaining the model's strong performance.

